Avoid Catastrophic Forgetting with Rank-1 Fisher from Diffusion Models

Catastrophic forgetting remains a central obstacle for continual learning in neural models. Popular approaches -- replay and elastic weight consolidation (EWC) -- have limitations: replay requires a strong generator and is prone to distributional drift, while EWC implicitly assumes a shared optimum across tasks and typically uses a diagonal Fisher approximation. In this work, we study the gradient geometry of diffusion models, which can already produce high-quality replay data. We provide theoretical and empirical evidence that, in the low signal-to-noise ratio (SNR) regime, per-sample gradients become strongly collinear, yielding an empirical Fisher that is effectively rank-1 and aligned with the mean gradient. Leveraging this structure, we propose a rank-1 variant of EWC that is as cheap as the diagonal approximation yet captures the dominant curvature direction. We pair this penalty with a replay-based approach to encourage parameter sharing across tasks while mitigating drift. On class-incremental image generation datasets (MNIST, FashionMNIST, CIFAR-10, ImageNet-1k), our method consistently improves average FID and reduces forgetting relative to replay-only and diagonal-EWC baselines. In particular, forgetting is nearly eliminated on MNIST and FashionMNIST and is more than halved on ImageNet-1k. These results suggest that diffusion models admit an approximately rank-1 Fisher. With a better Fisher estimate, EWC becomes a strong complement to replay: replay encourages parameter sharing across tasks, while EWC effectively constrains replay-induced drift.

==> inputs/addi-implementation-datasets.tex <==
\section{Additional implementation details}
% \label{app:addi_imp_det}
\subsection{Implementation details for empirical analysis}
We use the label-conditioned UNet implementation from \textit{Huggingface} as our denoising network. The UNet employs three ResNet blocks with $16$ output channels in each downsampling block.
For training, we use a batch size of $128$ and a learning rate of $2\times10^{-4}$ with the Adam optimizer \citep{kingma2017adammethodstochasticoptimization}, and train for 200 epochs per task for each dataset.

Training was performed on a single Nvidia A100 40GB GPU, taking a total of 157 minutes. 

\subsection{Additional implementation details for continual learning experiments}
We employ a label-conditioned UNet implementation from \textit{HuggingFace} as our denoising network, retaining the default hyper-parameters.  
The architecture consists of four ResNet blocks, with $128$ output channels in the first down-sampling block and $256$ output channels in the remaining blocks.  
For sampling, we use a DDIM scheduler with $50$ sampling steps and $1000$ noising steps.  

We summarize our training hyperparameters in Table~\ref{tab:config}. Unless otherwise stated, the same settings are used across all datasets and tasks.  
We also provide the average runtime (including FID evaluation) for each dataset and method in Table~\ref{tab:runtime_gpu}.

\input{inputs/tables/appendix/config}
\input{inputs/tables/appendix/gpu_runtime_table}


% \subsection{Additional dataset details}
\section{Additional Dataset Details}
\label{app:datasets}

All datasets are resized or padded to $32\times32$ for consistency.  
Table~\ref{tab:dataset-details} summarizes their configurations.  

\input{inputs/tables/appendix/dataset-details}

\subsection{Dataset Descriptions and Task Splits}

\begin{description}[leftmargin=1.5cm,style=nextline]

\item[MNIST.] A dataset of handwritten digits ($0$–$9$) with $60{,}000$ training and $10{,}000$ test images. Each task contains two digit classes.\\
Task splits:  
$T_1=\{0,1\},\;
T_2=\{2,3\},\;
T_3=\{4,5\},\;
T_4=\{6,7\},\;
T_5=\{8,9\}$.

\item[Fashion MNIST.] A dataset of $10$ grayscale clothing categories (e.g., shirts, shoes, bags) with $60{,}000$ training and $10{,}000$ test images. Each task contains two categories.\\
Task splits:  
$T_1=\{0,1\},\;
T_2=\{2,3\},\;
T_3=\{4,5\},\;
T_4=\{6,7\},\;
T_5=\{8,9\}$.

\item[CIFAR-10.] A dataset of $32\times32$ RGB images across $10$ classes (e.g., animals, vehicles) with $50{,}000$ training and $10{,}000$ test images. Each task contains two classes.\\
Task splits:  
$T_1=\{0,1\},\;
T_2=\{2,3\},\;
T_3=\{4,5\},\;
T_4=\{6,7\},\;
T_5=\{8,9\}$.

\item[ImageNet-1k (downsampled).] A large-scale dataset with $1{,}000$ object categories and $1.28$ million training images. We use the $32\times32$ downsampled version for computational efficiency. Each task contains fifty classes.\\
Task splits:  
$T_1=\{0,\dots,49\},\;
T_2=\{50,\dots,99\},\;
\dots\;
T_{20}=\{950,\dots,999\}$.
\end{description}


==> inputs/addi-learning-curves.tex <==
\section{Additional results}

\subsection{Continual learning curves for each task}
In this appendix, we provide a comprehensive set of FID evaluation plots for all tasks across the datasets considered in our experiments. These plots illustrate the model’s performance on individual tasks and complement the quantitative results presented in the main paper.

% \subsubsection{MNIST}
\input{inputs/figures/appendix/mnist_fid_plots}

% ---------------- Fashion-MNIST ----------------
% \subsubsection{Fashion-MNIST}
\input{inputs/figures/appendix/fmnist_fid_plots}

% ---------------- CIFAR-10 ----------------
% \subsubsection{CIFAR-10}
\input{inputs/figures/appendix/cifar10_fid_plots}

% ---------------- ImageNet64 ----------------
% \subsubsection{ImageNet-1k}
\input{inputs/figures/appendix/imagenet_fid_plots}


























% \subsubsection{MNIST}
% \begin{center}
% \foreach \i in {0,...,4}{%
%   \begin{minipage}{0.19\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/appendix/mnist/eval_task\i.pdf}
%     \par Task \i
%   \end{minipage}%
% }
% \end{center}

% % ---------------- Fashion-MNIST ----------------
% \subsubsection{Fashion-MNIST}
% \begin{center}
% \foreach \i in {0,...,4}{%
%   \begin{minipage}{0.19\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/appendix/fmnist/eval_task\i.pdf}
%     \par Task \i
%   \end{minipage}%
% }
% \end{center}

% % ---------------- CIFAR-10 ----------------
% \subsubsection{CIFAR-10}
% \begin{center}
% \foreach \i in {0,...,4}{%
%   \begin{minipage}{0.19\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/appendix/cifar10/eval_task\i.pdf}
%     \par Task \i
%   \end{minipage}%
% }
% \end{center}

% % ---------------- ImageNet64 ----------------
% \subsubsection{ImageNet-1k}
% \begin{center}
% \foreach \i in {0,...,19}{%
%   \begin{minipage}{0.19\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/appendix/imagenet64/eval_task\i.pdf}
%     \par Task \i
%   \end{minipage}%
%   \ifnum\i=4 \par\fi
%   \ifnum\i=9 \par\fi
%   \ifnum\i=14 \par\fi
%   \ifnum\i=19 \par\fi
% }
% \end{center}

==> inputs/figures/f-norm.tex <==
\begin{wrapfigure}[12]{r}{0.45\textwidth} % [12]=reserve ~12 lines to avoid clipping
  \vspace{-\baselineskip}                 % nudge up so top aligns with text
  \centering
  \includegraphics[width=\linewidth]{plots/frobenius.pdf}
  \caption{Top 5 eigenvalues of $F(\theta)$ at each timestep (log-scale).}
  \label{fig:top-eig}
\end{wrapfigure}

==> inputs/limitation.tex <==
\section{Limitation}
